Some analysable instances of mu-synthesis

I describe a verifiable criterion for the solvability of the 2 by 2 spectral Nevanlinna-Pick problem with two interpolation points, and likewise for three other special cases of the mu-synthesis problem. The problem is to construct an analytic 2 by 2 matrix function F on the unit disc subject to a finite number of interpolation constraints and a bound on the cost function sup {mu(F(z)): |z| < 1}, where mu is an instance of the structured singular value of a 2 by 2 matrix.

==> spectralCF.tex <==
\section{The spectral Carath\'eodory-Fej\'er problem} \label{spectralCF}
This is the problem one obtains from the spectral Nevanlinna-Pick problem if one allows the interpolation points to coalesce at $0$.

{\em Given $k\times k$ matrices $V_0,V_1, \dots, V_n,$ find an analytic function $F: \D\to\C^{k\times k}$ such that
\beq\label{derivs}
F^{(j)}(0) = V_j \quad \mbox{ for } j=1,\dots, n
\eeq
and
\beq\label{specrad}
r(F(\la)) \leq 1 \quad \mbox{ for all } \la\in\D.
\eeq

